Helen: Maliciously Secure Coopetitive Learning for Linear Models

Many organizations wish to collaboratively train machine learning models on their combined datasets for a common benefit (e.g., better medical research, or fraud detection). However, they often cannot share their plaintext datasets due to privacy concerns and/or business competition. In this paper, we design and build Helen, a system that allows multiple parties to train a linear model without revealing their data, a setting we call coopetitive learning. Compared to prior secure training systems, Helen protects against a much stronger adversary who is malicious and can compromise m-1 out of m parties. Our evaluation shows that Helen can achieve up to five orders of magnitude of performance improvement when compared to training using an existing state-of-the-art secure multi-party computation framework.

==> background.tex <==

\section{Background}

In this section, we provide a brief overview of the primitives used in \sys.

\subsection{Cryptographic building blocks}
\subsubsection{Threshold partially homomorphic encryption}
A partially homomorphic encryption scheme is a public key encryption scheme that allows limited computing on ciphertext.
For example, Paillier~\cite{Paillier} is an additive encryption scheme: multiplying two ciphertexts together generates a new ciphertext such that its decryption gives the sum of the two original plaintexts.
Any party with the public key can encrypt ciphertexts as well as performing ciphertext manipulations.

A \emph{threshold} variant of such a scheme has some additional properties.
While the public key is known to everyone, the secret key is split across a set of parties such that a subset of them must participate together to decrypt a ciphertext.
If not enough members participate, the ciphertext cannot be decrypted.
The threshold structure can be altered based on the adversary assumption.
In \sys, we use a threshold structure such that all parties must participate in order to decrypt a ciphertext because we also assume that an attacker can compromise $n-1$ out of $n$ parties.

\subsubsection{Zero knowledge proofs}
\sys also uses Schnorr like proofs to prove properties of the encrypted ciphers.
The two main building blocks we use are plaintext-ciphertext multiplication proof and ciphertext interval proof.
This is directly taken from~\cite{cramer2001multiparty} so we call it the CDN protocol. 
The protocol is an honest verifier zero knowledge protocol, but can be transformed into full zero-knowledge using existing techniques~\cite{garay2003strengthening,fiatshamir}.
See~\ref{paillier:matmul:proof:proof} for a description of the proof.

\subsubsection{Malicious MPC}
We utilize SPDZ~\cite{spdz}, a state of the art malicious MPC protocol, for both \sys and the evaluation baseline.
Another recent malicious MPC is authenticated garbled circuits~\cite{wang2017global}.
We decided to use SPDZ for our baseline because the majority of the computation in SGD is spent doing matrix multiplication, which is not efficiently represented in garbled circuits.
\wz{Is this a good enough reason?}

For the rest of this section we give an overview of the properties of SPDZ.
%
The input $a \in \mathds{F}_{p^{k}}$ to SPDZ is represented as $\langle a \rangle = (\delta, (a_1, \dots, a_n), (\gamma(a)_1, \dots, \gamma(a)_n))$.
We have that $a = \sum_i a_i$ and $\alpha(a + \delta) = \sum_i \gamma(a)_i$.
Each player holds $a_i, \gamma(a)_i$, and $\delta$ is public. 
$\gamma(a)$ is the MAC authenticating $a$ under a global key $\alpha$.

$\alpha$ is not revealed at the end of the protocol; otherwise the malicious parties can use $\alpha$ to construct new MACs.
The preprocessing phase generates 
\begin{align*}
\langle \alpha \rangle = ((\alpha_1, \dots, \alpha_n), (\beta_i, \gamma(\alpha)_1^{i}, \dots, \gamma(\alpha)_n^{i})_{i=1,\dots,n})
\end{align*}
where $\alpha = \sum_i \alpha_i$ and $\sum_j \gamma(\alpha)_i^{j} = \alpha \beta_i$.
% Player $i$ holds $\alpha_i, \beta_i, \gamma(\alph)_1^{i}, \dots, \gamma(\alpha)_n^{i}$.
% Each player $j$ sends player $i$ $\alpha_j$, as well as $\gamma(\alpha)_i^{j}$.
% Therefore, player $i$ will receive $\gamma(\alpha)_i^{j}$ and check that $\sum_j \gamma(\alpha)_i^{j} = \alpha \beta_i$.
At the end, $\alpha$ is revealed and verified by each party.

Since each shared value needs to satisfy $\sum_i \gamma(x)_i = \alpha(x + \delta)$, we know that this must hold true for the inputs as well.
Let $\vec{x}$ be the vector input to the SPDZ protocol.
Each element $\vec{x}_i$ is secret shared for each party $j$ such that $\vec{x}_i = \vec{x}_i^{j}$.

We augment the output check phase with a check of the input via our commitment scheme.
For a single element $x \in \mathds{Z}_p$.
Commit to $\com{x}$ and calculate $\com{\delta}$.
Also commit to $\com{\gamma(x)_i}$.
After release of $\alpha$, it must be true that $\alpha (\com{x} \cdot \com{\delta}) = \prod \com{\gamma(x)_i}$.

\subsection{Learning and Convex Optimization}

% \begin{center}
%   \begin{picture}(400,200)(10,100)

%     \put(10, 200){\framebox(50,50)[c]{Party i}}

%     \put(320, 200){\framebox(50,50)[c]{Master}}
    
%     \put(150, 250){Step 2: $x_{i}^{k+1}, u_{i}^{k}$}
%     \put(130, 240){\vector(1,0){120}}

%     \put(150, 210){Step 4: $z^{k+1}$}
%     \put(250, 200){\vector(-1,0){120}}

%     \put(10, 150){Step 1: $x_{i}^{k+1} = f(u_{i}^{k}, z^{k})$}
%     \put(10, 120){Step 5: $u_{i}^{k+1} = h(x_{i}^{k+1}, z^{k+1})$}

%     \put(280, 150){Step 3: $z^{k+1} = g(\sum x_{i}^{k+1}, \sum u_{i}^{k})$}

%   \end{picture}
% \end{center}


Much of contemporary machine learning can be framed in the context of minimizing the \emph{cumulative error} (or loss) of a model over the training data. 
While there is considerable excitement around deep neural networks, the vast majority or real-world machine learning applications still rely on robust linear models.
When paired with the appropriate loss function (e.g., squared-error), linear models are well understood and can be efficiently and reliably learned using established convex optimization procedures. 
Furthermore, with the addition of a regularization function (e.g., $L^1$ regularization) these models can inform the selection of complex non-linear feature functions and fit high-dimensional data.


In this work, we focus on linear models with squared error and various forms of regularization resulting in the following family of optimization problems for the multiparty learning setting:
% \begin{equation}
% \hat{w} = \arg\min_w \sum_{j=1}^p \sum_{i=1}^{n_j} \left(x^{(j)}_i \cdot w - y^{(j)}_i\right)^2 + \lambda \mathbf{R}(w),\label{eqn:leastsquares}
% \end{equation}
\begin{equation}
\hat{\vec{w}} = \arg\min_w \frac{1}{2}\sum_{i=1}^p  \| \matr{X}_i \vec{w} - \vec{y}_i\|^2_2 + \lambda \mathbf{R}(\vec{w}),\label{eqn:leastsquares}
\end{equation}
where $\matr{X}_i \in \mathbb{R}^{n_i,d}$ and $\vec{y}_i \in \mathbb{R}^{n_i}$ are 
the training data (features and labels)
% the covariate matrix (features) and response vector (labels) 
from party $i$.  
The regularization function $\mathbf{R}$ and regularization tuning parameter $\lambda$ are used to improve prediction accuracy on high-dimensional data.  
Typically the regularization function takes one of the following forms:
\begin{align}
    \mathbf{R}_{L^1}(\vec{w}) & = \sum_{j=1}^d |\vec{w}_j|, &
    \mathbf{R}_{L^2}(\vec{w}) & = \frac{1}{2}\sum_{j=1}^d \vec{w}_j^2 \nonumber
\end{align}
corresponding to Lasso ($L^1$) and Ridge ($L^2$) regression respectively.
The estimated model $\hat{\vec{w}} \in \mathbb{R}^d$ can  then used to render a new prediction $\hat{y}_* = \hat{\vec{w}}^T \vec{x}_*$ at a query point $\vec{x}_*$,

\joey{Add a note about lasso and large $d$ and connect to basis pursuit.}

The optimization problem in Eq.~\ref{eqn:leastsquares} can be solved efficiently in the centralized setting using convex optimization algorithms.  
Furthermore, the gradient of the objective in Eq.~\ref{eqn:leastsquares} can be factored
% \begin{equation}
%     \nabla_\vec{w} J(\vec{w}) = \sum_{j=1}^p 2\left(\matr{X}_i \vec{w} - \vec{y}_i\right)^T \matr{X}_i + \lambda \nabla_\vec{w} \mathbf{R}(\vec{w})
% \end{equation}
across parties enabling distributed gradient descent.
However, directly applying distributed gradient descent would require many rounds of communication and coordination across the parties and would therefore be costly to support in the secure setting. 
In this work we explore an alternative approach to distributed optimization derived for settings where coordination and communication costs are high.  




\noindent\textbf{ADMM.} Alternating Direction Method of Multipliers (ADMM)~\cite{admmChapter} is an established technique for distributed convex optimization.  
The ADMM algorithm leverages Lagranian duality to decompose Eq.~\ref{eqn:leastsquares} into a sequence of independent sub-problems that can be efficiently solved without coordination.
In the following we give a high-level overview of the ADMM algorithm and introduce the details for the commonly used Lasso regression problem.

We reformulate the optimization problem in Eq.~\ref{eqn:leastsquares} by introducing \emph{additional} variables and constraints:
\begin{align}
 \underset{
 \{\vec{w}_i\}_{i=1}^p, \, \vec{z}
 }{\textbf{minimize:}}
  & \quad \frac{1}{2}\sum_{i=1}^p  
  \|\matr{X}_i \vec{w}_i - \vec{y}_i\|_2^2 + \lambda \mathbf{R}(\vec{z}),\nonumber \\
\textbf{such that: } &\quad \vec{w}_i = \vec{z} \text{ for all $i \in \{1,\ldots, p\}$} \label{eqn:constrainedobj}
\end{align}
In this equivalent formulation we have factored the optimization problem across each of the parties by allowing each party to estimate it's own model $\vec{w}_i$. 
However, we still require each of the $\vec{w}_i$ parameters are equivalent to the \emph{consensus model} $\vec{z} \in \mathbb{R}^d$.
We construct an \emph{augmented Langrangian} for the constrained optimization problem: 
% Eq.~\ref{eqn:constrainedobj}
\begin{align}
    & L\left(\{\vec{w}_i\}_{i=1}^p, \vec{z}, \vec{u}\right) = 
     \frac{1}{2}\sum_{i=1}^p  \|\matr{X}_i \vec{w}_i - \vec{y}_i\|_2^2 + \lambda \mathbf{R}(\vec{z}) + \nonumber \\
    & \quad\quad \rho\sum_{i=1}^p \vec{u}_i^T \left(\vec{w}_i  - \vec{z}\right) +
    \frac{\rho}{2}\sum_{i=1}^p \left|\left|\vec{w}_i  - \vec{z}\right|\right|_2^2 \label{eqn:lagrangian}
\end{align}
where the dual vectors $\vec{u}_i \in \mathbb{R}^d$ capture the mismatch between the model estimated by party $i$ and the shared model $\vec{z}$ and the augmenting term $\frac{\rho}{2}\sum_{i=1}^p \left|\left|\vec{w}_i  - \vec{z}\right|\right|_2^2$ adds an additional penalty (scaled by the constant $\rho$) for deviating from consensus model $\vec{z}$.
% Note that this augmenting penalty vanishes when consensus is achieved and all $\vec{w}_i = \vec{z}$.

The ADMM algorithm is a simple iterative dual ascent on the augmented Langranian (Eq.~\ref{eqn:lagrangian}).  
On the $k^{\text th}$ iteration, each party locally solves this closed-form expression:
% \begin{align*}
%     \vec{w}_i^{k+1} & \leftarrow \arg \min_{\vec{w}_i}  \left(\matr{X}_i \vec{w}_i - \vec{y}_i\right)^2 + \vec{w}_i^T \vec{u}_i^{k}  + \frac{\rho}{2}||\vec{w}_i - \vec{z}^k||_2^2
% \end{align*}

\begin{equation}
    \vec{w}_i^{k+1} \leftarrow \left(\matr{X}_i^T \matr{X}_i + \rho \matr{I}\right)^{-1} 
    \left( \matr{X}_i^T \vec{y}_i + \rho \left(\vec{z}^k  - \vec{u}_i^k\right)\right) \label{eq:primalupdate}
\end{equation}
and then shares its local model $\vec{w}_i^{k+1}$ and Lagrange multipliers $\vec{u}_i^{k}$ to solve for the new consensus parameters


% \begin{align*}
%     \vec{z}^{k+1} & \leftarrow \arg \min_{\vec{z}}  \lambda \mathbf{R}(\vec{z}) + \sum_{i=1}^p \vec{z}^T \vec{u}_i^{k}  + \frac{\rho}{2}\sum_{i=1}^p||\vec{w}_i^{k+1} - \vec{z}||_2^2.
% \end{align*}
\begin{align}
    \vec{z}^{k+1} & \leftarrow \arg \min_{\vec{z}}  \lambda \mathbf{R}(\vec{z}) +  \frac{\rho}{2}\sum_{i=1}^p||\vec{w}_i^{k+1} - \vec{z} + \vec{u}_i^{k} ||_2^2. \label{eq:zupdate}
\end{align}
Finally, each party uses the new consensus parameters $\vec{z}^{k+1}$ to update its local Lagrange multipliers
\begin{align}
    \vec{u}_i^{k+1} & \leftarrow \vec{u}_i^{k} + \vec{w}_i^{k+1} - \vec{z}^{k+1} .\label{eq:dualupdate}
\end{align}


%Similarly, the ridge regression ($L^2$-regularization) consensus update is given by:
%\begin{equation}
%\vec{z}^{k+1} \leftarrow \left(\frac{\rho}{\lambda + p \rho}\right) \sum_{i=1}^p\left( \vec{w}^{k+1}_i - \vec{u}^{k}_i\right)\label{eq:l2consensus}
%\end{equation}
The consensus update equations depend on the local models $\vec{w}_i$ and Lagrange multipliers $\vec{u}_i$ through their \emph{summation}, which is essential to an efficient MPC formulation. 
%
The update equations \eqref{eq:primalupdate}, \eqref{eq:zupdate}, and \eqref{eq:dualupdate} are executed iteratively until all updates reach a fixed point.  
In practice, a relatively large fixed number of iterations may be used as a stopping condition, and that is what we do in \sys.

\subsubsection{LASSO}
\label{sec:trainingtask}
\newcommand{\shared}[1]{\textcolor{blue}{#1}}

We use LASSO as a running example for the rest of the paper, and we use the specific equations to illustrate how our secure training protocol works.
LASSO is a popular regularized linear regression model that uses L1 as the regularizer.
The LASSO formulation is given by the optimization objective $\argmin_{\vec{w}} \| \matr{X} \vec{w} - \vec{y}\|_{2}^{2} + \lambda \| \vec{w} \|$.
\cref{fig:lasso} shows the ADMM training procedure for LASSO.

% For LASSO  ($L^1$-regularization) update is given by:
% \begin{align}
%     \vec{z}^{k+1} \leftarrow 
%     S_{\lambda/p\rho}
%     \left(\frac{1}{p}\sum_{i=1}^p \left(w_i^{k+1} + u_i^{k} \right) \right) \label{eq:l1consensus}
% \end{align}
% where $S_\kappa(a)$ 
% % $= (1 - \kappa/|a|)_+a$


\begin{framed}
\label{fig:lasso}
\underline{The federated learning task for LASSO} 


\medskip

\noindent Input of party $P_i$: $X_i, \vec{y}_i$


\begin{enumerate}
\item $A_i \gets  \left(\matr{X}_i^T \matr{X}_i + \rho \matr{I}\right)^{-1} $

\item $\vec{b}_i \gets \matr{X}_i^T \vec{y}_i $

\item $\vec{u^0}, \vec{z^0}, \vec{w^0} \gets \vec{0}$

\item {\tt For} $k = 0$, {\tt ADMMIterations}-1:

\begin{enumerate}
\item  $\shared{\vec{w}_i^{k+1}} \leftarrow  A_i (\vec{b}_i + \rho \left(\shared{\vec{z}^k}  - \shared{\vec{u}_i^k}\right))$
  
\item   $\shared{\vec{z}^{k+1}} \leftarrow 
    S_{\lambda/p\rho}
    \left(\frac{1}{p}\sum_{i=1}^p \left(\shared{\vec{w}_i^{k+1}} + \shared{\vec{u}_i^{k}} \right) \right)$ 


\item    $\shared{\vec{u}_i^{k+1}}  \leftarrow \shared{\vec{u}_i^{k}} + \shared{\vec{w}_i^{k+1}} - \shared{\vec{z}^{k+1}}$ 
\end{enumerate}
\end{enumerate}

\end{framed}

$S_{\lambda/p\rho}$ is the soft the soft thresholding operator, which is defined as
\begin{equation}
S_{\kappa}(a)=
\begin{cases}
a - \kappa & a > \kappa\\
0 & |a| \leq \kappa \\
a + \kappa & a < -\kappa
\end{cases} \label{eq:softthreshold}
\end{equation}

The quantities in \shared{color} are quantities that are intermediate values in the computation, whereas the quantities in black are values known to one party. We will refer back to this distinction in the technical sections.


\eat{

\justforus{
The first line specifies an optimization problem is executed at each party locally with no interaction.
The second line requires coordination among all the parties, and is executed via an MPC protocol.
The third line is the result that is passed to every party at the end of MPC and computed locally.
}

\justforus{
The original ADDM formulation written by Joey:

\begin{align}
    \vec{w}_i^{k+1} & \leftarrow \arg \min_{\vec{w}}  
    \left(\matr{X}_i \vec{w} - \vec{y}_i\right)^2 
    +
    \rho||\vec{w} - \vec{z}^k + \vec{u}_i^{k} ||_2^2 
\end{align}

}
}





% In this section, we present the ADMM formulation of $L^1$-regularized linear regression (LASSO) we use in our experimental evaluation.
% Each party $i$ has a dataset consisting of features $\matr{X}_i$ and labels $\vec{y}_i$
% \begin{align*}
% \min_{\vec{w}_i} \| X_i \vec{w}_i - \vec{y}_i \|_{2}^{2} + \lambda |\vec{w}|
% \end{align*}

% This can be expressed as a constrained problem
% \begin{align*}
% \min_{\vec{w}_i} \sum_{i=1}^{n} \| X_i \vec{w}_i - \vec{y}_i \|_{2}^{2} + \lambda \| \vec{z} \|_1\\
% \text{subject to } \vec{w}_i = \vec{z} = 0 \text{ for } i = 1 \dots n
% \end{align*}

% To solve this, we can take the augmented Lagrangian
% \begin{align*}
% L_{p}(\vec{w}_i, \vec{z}, \vec{v}_i) &= \| X_i \vec{w}_i - \vec{y}_i \|_{2}^{2} + \lambda \| \vec{z} \|_1 + \\
% &\dfrac{\rho}{2} \| \vec{w}_i - \vec{z} + \vec{u}_i \|_{2}^{2} - \dfrac{\rho}{2}\| \vec{u}_i\|_{2}^{2}
% \end{align*}

% This reduces to the following iterative solution:

% \begin{align*}
% \vec{w}_{i}^{k+1} &= \text{argmin}_{\vec{w}_{i}} \dfrac{1}{2} \| X_{i} \vec{w}_{i} - \vec{y}_{i}\|_{2}^{2} + \dfrac{\rho}{2} \|\vec{w}_{i} - \vec{z}^{k} + \vec{u}_{i}^{k}\|_{2}^{2}\}\\
% \vec{z}^{k+1} &= S_{\lambda / \rho N}(\bar{\vec{w}}^{k+1} + \bar{\vec{u}}^{k}) \\
% \vec{u}_{i}^{k+1} &= \vec{u}_{i}^{k} + \vec{w}_{i}^{k+1} - \vec{z}^{k+1} 
% \end{align*}




